Believing is Seeing: Unobserved Object Detection using Generative Models

Can objects that are not visible in an image -- but are in the vicinity of the camera -- be detected? This study introduces the novel tasks of 2D, 2.5D and 3D unobserved object detection for predicting the location of nearby objects that are occluded or lie outside the image frame. We adapt several state-of-the-art pre-trained generative models to address this task, including 2D and 3D diffusion models and vision-language models, and show that they can be used to infer the presence of objects that are not directly observed. To benchmark this task, we propose a suite of metrics that capture different aspects of performance. Our empirical evaluation on indoor scenes from the RealEstate10k and NYU Depth v2 datasets demonstrate results that motivate the use of generative models for the unobserved object detection task.

==> rebut_fig.tex <==
\begin{figure*}[!b]
    \vspace{-1em}
    \centering
    \rotatebox[origin=l]{90}{\footnotesize CAR}
    \begin{subfigure}[]{0.27\linewidth}
        \centering
        \begin{tikzpicture}
            \node [anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=\linewidth]{rebutter.png}};
            \draw[white, thick, dashed] (0.22*\linewidth, 0.01) -- (0.22*\linewidth, 0.5648*\linewidth);
            \draw[white, thick, dashed] (0.78*\linewidth, 0.01) -- (0.78*\linewidth, 0.5648*\linewidth);
        \end{tikzpicture}
        \caption{$\inim$ (center) and $\outim$ (full)}
    \end{subfigure}
    \begin{subfigure}[]{0.15\linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebut_DFM.png}
        \caption{DFM-based $\sd^\text{3D}$}
    \end{subfigure}
    \begin{subfigure}[]{0.27\linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebut_car.png}
        \caption{SDXL-based $\sd^\text{2D}$}
    \end{subfigure}
    \begin{subfigure}[]{0.27\linewidth}
        \centering
        \includegraphics[width=\linewidth]{rebut_f.png}
        \caption{ChatGPT-4o-based $\sd^\text{2D}$}
    \end{subfigure}
    \vspace{-1em}
    {\tt 0}\ \includegraphics[width=0.5\linewidth, trim={12pt 8pt 10pt 8pt}, clip]{images/plasma_scale.pdf}\ {\tt 1}
    \caption{Results for an outdoor scene--object pair. The GT position is denoted by a white star.}
    \label{fig:1}
    \vspace{-1em}
\end{figure*}

==> sections/archived_tables/table2.tex <==
% \begin{table*}[!t]\centering
% \renewcommand{\arraystretch}{1.0}
% \caption{
% Performance of all models on the 2.5D and 3D \task tasks in the \rk and \nyu datasets have been tabulated.
% We report the normalized cross-entropy $\cent$, the normalized nearest neighbor distance $\dnn$, the percentage of false negatives ($\falseneg$), the prediction entropy $\ent$ and the region-wise classification accuracy $\rwa$.
% The best non-baseline result is indicated in bold.
% }
% \vskip 1ex
% \label{tab:3D}
% \begin{tabularx}{\linewidth}{@{}l CCCC | CCCC@{}}
% \toprule
% & \multicolumn{4}{c|}{\textbf{2.5D Task: \rk}} & \multicolumn{4}{c}{\textbf{3D Task: \rk}} \\
% \midrule
% \textbf{Methods} & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ \\
% \midrule
% Baseline-uniform & $1.72$ & $0.00$ & $0.00$ & $1.00$ & $2.32$ & $0.00$ & $0.00$ & $1.00$ \\
% Baseline-oracle & ${0.00}$ & ${0.00}$ & ${0.00}$ & ${0.24}$ & $3.11$ & $19.84$ & $43.75$ & $0.71$ \\
% \midrule
% DFM ($n_s=25, k=4$) & $\mathbf{0.15}$ & $\mathbf{1.18}$ & $\mathbf{0.00}$ & $\mathbf{0.74}$ & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ \\
% DFM ($n_s=25, k=3$) & $0.18$ & $2.17$ & $0.21$ & $0.83$ & $2.14$ & $3.11$ & $31.72$ & $0.47$ \\
% DFM ($n_s=25, k=2$) & $1.71$ & $2.45$ & $0.28$ & $0.88$ & $2.77$ & $6.32$ & $36.85$ & $0.54$ \\
% DFM ($n_s=15, k=4$) & $2.04$ & $1.55$ & $2.27$ & $0.77$ & $2.98$ & $0.14$ & $33.45$ & $0.50$ \\
% DFM ($n_s=10, k=4$) & $2.82$ & $6.13$ & $8.12$ & $0.82$ & $4.33$ & $1.89$ & $45.12$ & $0.62$ \\
% \midrule
% SDXL (w/ obj prompts) & $1.48$ & $9.04$ & $2.63$ & $0.82$ & -- & -- & -- & -- \\
% SDXL (w/o obj prompts) & $2.48$ & $7.86$ & $31.58$ & $0.86$ & -- & -- & -- & -- \\
% SDXL (w/o prompts) & $8.25$ & $13.23$ & $86.32$ & $0.94$ & -- & -- & -- & -- \\
% \bottomrule
% \end{tabularx}
% \end{table*}

% %%%%%%%%%% NYU %%%%%%%%%%%

% \begin{table*}[!t]\centering
% \renewcommand{\arraystretch}{1.0}
% \caption{
% Performance of all models on the 2.5D and 3D \task tasks in the \nyu dataset.
% }
% \vskip 1ex
% \label{tab:3D_NYU}
% \begin{tabularx}{\linewidth}{@{}l CCCCC | CCCC@{}}
% \toprule
% & \multicolumn{5}{c|}{\textbf{2.5D Task: \nyu}} & \multicolumn{4}{c}{\textbf{3D Task: \nyu}} \\
% \midrule
% \textbf{Methods} & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ & $\rwa \uparrow$ & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ \\
% \midrule
% Baseline-uniform & $1.72$ & $0.00$ & $0.00$ & $1.00$ & $0.08$ & $2.32$ & $0.00$ & $0.00$ & $1.00$ \\
% Baseline-oracle & ${0.00}$ & ${0.00}$ & ${0.00}$ & ${0.24}$ & ${1.00}$ & $3.11$ & $19.84$ & $43.75$ & $0.71$ \\
% \midrule
% DFM ($n_s=25, k=4$) & $\mathbf{0.15}$ & $\mathbf{1.18}$ & $\mathbf{0.00}$ & $\mathbf{0.74}$ & $0.38$ & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ \\
% DFM ($n_s=25, k=3$) & $0.18$ & $2.17$ & $0.21$ & $0.83$ & $0.34$ & $2.14$ & $3.11$ & $31.72$ & $0.47$ \\
% DFM ($n_s=25, k=2$) & $1.71$ & $2.45$ & $0.28$ & $0.88$ & $0.35$ & $2.77$ & $6.32$ & $36.85$ & $0.54$ \\
% DFM ($n_s=15, k=4$) & $2.04$ & $1.55$ & $2.27$ & $0.77$ & $0.19$ & $2.98$ & $0.14$ & $33.45$ & $0.50$ \\
% DFM ($n_s=10, k=4$) & $2.82$ & $6.13$ & $8.12$ & $0.82$ & $0.11$ & $4.33$ & $1.89$ & $45.12$ & $0.62$ \\
% \midrule
% SDXL (w/ obj prompts) & $1.48$ & $9.04$ & $2.63$ & $0.82$ & $\mathbf{0.47}$ & -- & -- & -- & -- \\
% SDXL (w/o obj prompts) & $2.48$ & $7.86$ & $31.58$ & $0.86$ & $0.28$ & -- & -- & -- & -- \\
% SDXL (w/o prompts) & $8.25$ & $13.23$ & $86.32$ & $0.94$ & $0.12$ & -- & -- & -- & -- \\
% \bottomrule
% \end{tabularx}
% \end{table*}

% 2.5D task
% \begin{table*}[t]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \caption{
% Performance of all models on the 2.5D task in the \rk and \nyu datasets.
% We report the normalized cross-entropy $\cent$, the normalized nearest neighbor distance $\dnn$, the percentage of false negatives ($\falseneg$), and the prediction entropy $\ent$.
% The best non-baseline result is indicated in bold.
% }
% \vskip 1ex
% \label{tab:2.5D}
% \begin{tabularx}{\textwidth}{@{}l XXXX | XXXX @{}}
% \toprule
% & \multicolumn{4}{c }{\textbf{\rk}} & \multicolumn{4}{c}{\textbf{\nyu}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \textbf{Methods} & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ \\
% \midrule
% Baseline-uniform & $1.72$ & $0.00$ & $0.00$ & $1.00$ & $1.72$ & $0.00$ & $0.00$ & $1.00$ \\
% Baseline-oracle & ${0.00}$ & ${0.00}$ & ${0.00}$ & ${0.24}$ & ${0.00}$ & ${0.00}$ & ${0.00}$ & ${0.24}$ \\
% \midrule
% DFM ($n_s=25, k=4$) & $\mathbf{0.15}$ & $\mathbf{1.18}$ & $\mathbf{0.00}$ & $\mathbf{0.74}$ & $\mathbf{0.15}$ & $\mathbf{1.18}$ & $\mathbf{0.00}$ & $\mathbf{0.74}$ \\
% DFM ($n_s=25, k=3$) & $0.18$ & $2.17$ & $0.21$ & $0.83$ & $0.18$ & $2.17$ & $0.21$ & $0.83$ \\
% DFM ($n_s=25, k=2$) & $1.71$ & $2.45$ & $0.28$ & $0.88$ & $1.71$ & $2.45$ & $0.28$ & $0.88$ \\
% DFM ($n_s=15, k=4$) & $2.04$ & $1.55$ & $2.27$ & $0.77$ & $2.04$ & $1.55$ & $2.27$ & $0.77$ \\
% DFM ($n_s=10, k=4$) & $2.82$ & $6.13$ & $8.12$ & $0.82$ & $2.82$ & $6.13$ & $8.12$ & $0.82$ \\
% \midrule
% SDXL (w/ obj prompts) & $1.48$ & $9.04$ & $2.63$ & $0.82$ & $1.48$ & $9.04$ & $2.63$ & $0.82$ \\
% SDXL (w/o obj prompts) & $2.48$ & $7.86$ & $31.58$ & $0.86$ & $2.48$ & $7.86$ & $31.58$ & $0.86$ \\
% SDXL (w/o prompts) & $8.25$ & $13.23$ & $86.32$ & $0.94$ & $8.25$ & $13.23$ & $86.32$ & $0.94$ \\
% \bottomrule
% \end{tabularx}
% \end{table*}





==> sections/archived_tables/table3.tex <==
% \begin{table*}[t]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \caption{
% Performance of all models on the 3D task in the \rk and \nyu datasets.
% }
% \vskip 1ex
% \label{tab:3D}
% \begin{tabularx}{\textwidth}{@{}l XXXX | XXXX @{}}
% \toprule
% & \multicolumn{4}{c}{\textbf{\rk}} & \multicolumn{4}{c}{\textbf{\nyu}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \textbf{Methods} & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ \\
% \midrule
% Baseline-uniform & $2.32$ & $0.00$ & $0.00$ & $1.00$ & $2.32$ & $0.00$ & $0.00$ & $1.00$ \\
% Baseline-oracle & $3.11$ & $19.84$ & $43.75$ & $0.71$ & $3.11$ & $19.84$ & $43.75$ & $0.71$ \\
% \midrule
% DFM ($n_s=25, k=4$) & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ \\
% DFM ($n_s=25, k=3$) & $2.14$ & $3.11$ & $31.72$ & $0.47$ & $2.14$ & $3.11$ & $31.72$ & $0.47$ \\
% DFM ($n_s=25, k=2$) & $2.77$ & $6.32$ & $36.85$ & $0.54$ & $2.77$ & $6.32$ & $36.85$ & $0.54$ \\
% DFM ($n_s=15, k=4$) & $2.98$ & $0.14$ & $33.45$ & $0.50$ & $2.98$ & $0.14$ & $33.45$ & $0.50$ \\
% DFM ($n_s=10, k=4$) & $4.33$ & $1.89$ & $45.12$ & $0.62$ & $4.33$ & $1.89$ & $45.12$ & $0.62$ \\
% \bottomrule
% \end{tabularx}
% \end{table*}


% \begin{table*}[t]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \caption{
% Performance of all models on the 3D task in the \rk and \nyu datasets.
% }
% \vskip 1ex
% \label{tab:3D}
% \begin{tabularx}{\textwidth}{@{}l XXXX | XXXX @{}}
% \toprule
% & \multicolumn{4}{c}{\textbf{\rk}} & \multicolumn{4}{c}{\textbf{\nyu}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \textbf{Methods} & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ & $\cent \downarrow$ & $\dnn\% \downarrow$ & $\falseneg\% \downarrow$ & $\ent \downarrow$ \\
% \midrule
% Baseline-uniform & $2.32$ & $0.00$ & $0.00$ & $1.00$ & $2.32$ & $0.00$ & $0.00$ & $1.00$ \\
% Baseline-oracle & $3.11$ & $19.84$ & $43.75$ & $0.71$ & $3.11$ & $19.84$ & $43.75$ & $0.71$ \\
% \midrule
% DFM ($n_s=25, k=4$) & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ & $\mathbf{1.66}$ & $\mathbf{0.03}$ & $\mathbf{12.75}$ & $\mathbf{0.43}$ \\
% \bottomrule
% \end{tabularx}
% \end{table*}

==> sections/extra.tex <==
% \begin{figure}[!t]
%     \centering
    % \subfloat[]{%
    %    \includegraphics[width=0.32\linewidth]{./images/dfm-poses.tex}%
    %    \label{fig:dfm-poses}%
    % } 
    % \hfill
    % \subfloat[]{%
    %    \includegraphics[width=0.28\linewidth]{./images/sdxl-samples.tex}%
    %    \label{fig:sdxl-samples}%
    %     % \vspace{17pt}
    %     \vspace{8.5pt}
    % }
    % \hfill
    % \subfloat[]{%
    %    \includegraphics[width=0.28\linewidth]{./images/vlm-samples.tex}%
    %    \label{fig:vlm-samples}%
    %     % \vspace{22pt}
    %     \vspace{11pt}
    % }
    % \includegraphics[width=\linewidth]{./images/combined-methods-samples.tex}
    % \includegraphics[width=\linewidth]{./images/dfm-poses.tex}
    % \includegraphics[width=\linewidth]{./images/sdxl-pipeline.tex}
    % \includegraphics[width=\linewidth]{./images/vlm-pipeline.tex}
    % \vspace{-0.25in}
    % \caption{The sampling processes in our proposed detection pipelines.
    % (a)~The 3D diffusion pipeline uses $k$ camera poses to generate $n_s$ samples, which are combined to produce $\sd^\text{3D}$.
    % \caption{The 3D diffusion pipeline uses $k=4$ camera poses to generate $n_s=$ samples, which are combined to produce $\sd^\text{3D}$.}
    % (b)~The 2D diffusion pipeline uses outpainting to generate $n_s$ expanded images, which are combined to produce $\sd^\text{2D}$.
    % (c)~The Vision--Language Model (VLM) pipeline answers $n_s$ expanded region-wise queries to obtain $\sd^\text{2D}$.
    % These pipelines highlight distinct approaches for probabilistic object detection in 2D and 3D spaces.}
%     \label{fig:pipelines}
%      \vspace{-0.1in}
% \end{figure}

% \begin{table*}
% \centering
% \begin{tabular}{lccccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ & $\rwa\uparrow$ \\
% \hline
% DFM ($n_s = 25, k=4$) & 1.555 ± 1.460 & 0.774 ± 0.119 & 5.990 ± 39.470 & 3.226\% & 0.747 ± 0.139 \\
% DFM ($n_{s}=25, k=3$) & 1.877 ± 1.327 & 0.818 ± 0.112 & 18.136 ± 32.482 & 12.11\% & 0.626 ± 0.107 \\
% DFM ($n_{s}=25, k=2$) & 2.328 ± 1.041 & 0.902 ± 0.067 & 14.037 ± 42.005 & 86.84\% & 0.581 ± 0.182 \\
% \midrule
% DFM ($n_{s}=15, k=4$) & 1.736 ± 0.414 & 0.898 ± 0.117 & 15.334 ± 23.380 & 60.53\% & 0.573 ± 0.198  \\
% DFM ($n_{s}=10, k=4$) & 2.247 ± 1.206 & 0.923 ± 0.014 & 14.082 ± 29.083 & 71.05\% & 0.550 ± 0.337 \\
% \hline
% \end{tabular}
% \caption{2D Metrics for \rk\ with lower number of poses and samples, used to study the trend}
% \label{table:ablations_Re10k_2D}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lccccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ & $\rwa\uparrow$ \\
% \hline
% DFM ($n_{s}=25, k=4$) & 1.661 ± 1.336 & 0.696 ± 0.128 & 6.217 ± 36.112 & 5.556\% & 0.765 ± 0.236 \\
% DFM ($n_{s}=25, k=3$) & 2.053 ± 0.351 & 0.929 ± 0.145 & 20.459 ± 35.216 & 17.29\% & 0.589 ± 0.340 \\
% DFM ($n_{s}=25, k=2$) & 2.691 ± 1.187 & 0.978 ± 0.072 & 15.871 ± 45.028 & 89.96\% & 0.545 ± 0.190 \\
% \midrule
% DFM ($n_{s}=15, k=4$) & 1.915 ± 0.497 & 0.969 ± 0.030 & 17.242 ± 25.764 & 55.80\% & 0.623 ± 0.353 \\
% DFM ($n_{s}=10, k=4$) & 2.498 ± 1.354 & 0.998 ± 0.012 & 15.936 ± 31.011 & 73.92\% & 0.614 ± 0.356 \\
% \hline
% \end{tabular}
% \caption{2D Metrics for \nyu\ with lower number of poses and samples, used to study the trend}
% \label{table:ablations_nyu_2D}
% \end{table*}

% %%%%%%%%%%%%%% 2.5D %%%%%%%%%%%%%%%%%%

% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% DFM ($n_{s}=25, k=4$) & 1.955 ± 1.033 & 0.530 ± 0.441 & 5.128 ± 3.042 & 3.226\% \\
% DFM ($n_{s}=25, k=3$) & 2.018 ± 0.053 & 0.814 ± 0.080 & 12.889 ± 1.067 & 12.110\% \\
% DFM ($n_{s}=25, k=2$) & 2.586 ± 2.650 & 0.996 ± 0.003 & 13.461 ± 1.552 & 86.845\% \\
% \midrule
% DFM ($n_{s}=15, k=4$) & 2.113 ± 0.778 & 0.877 ± 0.067 & 9.018 ± 6.332 & 60.537\% \\
% DFM ($n_{s}=10, k=4$) & 2.498 ± 1.354 & 0.997 ± 0.002 & 18.018 ± 9.607 & 71.050\% \\
% \hline
% \end{tabular}
% \caption{2.5D Metrics for \rk\ with lower number of poses and samples, used to study the trend}
% \label{table:ablations_Re10k_2.5D}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% DFM ($n_{s}=25, k=4$) & 1.785 ± 2.101 & 0.610 ± 0.207 & 4.214 ± 2.803 & 5.556\% \\
% DFM ($n_{s}=25, k=3$) & 2.067 ± 0.093 & 0.798 ± 0.089 & 11.442 ± 1.305 & 15.230\% \\
% DFM ($n_{s}=25, k=2$) & 2.523 ± 2.301 & 0.990 ± 0.005 & 12.786 ± 1.781 & 83.658\% \\
% \midrule
% DFM ($n_{s}=15, k=4$) & 2.184 ± 0.652 & 0.867 ± 0.079 & 8.336 ± 6.174 & 77.246\% \\
% DFM ($n_{s}=10, k=4$) & 2.451 ± 1.231 & 0.995 ± 0.003 & 17.124 ± 9.403 & 80.827\% \\
% \hline
% \end{tabular}
% \caption{2.5D Metrics for \nyu\ with lower number of poses and samples, used to study the trend}
% \label{table:ablations_NYU_2.5D}
% \end{table*}

% %%%%%%%%%%% Outpainting 2D %%%%%%%%%%%%
% \begin{table*}
% \centering
% \begin{tabular}{lccccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ & $\rwa\uparrow$ \\
% \hline
% SDXL w/ object cues & $1.257 \pm 2.033$ & $0.848 \pm 0.150$ & $0.446 \pm 25.490$ & $3.846\%$ & $0.918 \pm 0.147$ \\
% SDXL w/o object cues & $1.888 \pm 1.904$ & $0.882 \pm 0.115$ & $6.274 \pm 14.890$ & $55.409\%$ & $0.688 \pm 0.272$ \\
% SDXL w/o prompts & $2.583 \pm 4.612$ & $0.887 \pm 0.106$ & $6.901 \pm 12.663$ & $58.927\%$ & $0.773 \pm 0.276$ \\
% \hline
% \end{tabular}
% \caption{Comparison of metrics across different SDXL 2D methods: with object prompts, no cues, and no prompts for the \rk dataset.}
% \label{table:SDXL_ablations_2D_Re10k}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lccccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$& $\falseneg \downarrow$ & $\rwa\uparrow$ \\
% \hline
% SDXL w/ object cues & $1.223 \pm 2.107$ & $0.778 \pm 0.212$ & $0.510 \pm 26.929$ & $5.438\%$ & $0.944 \pm 0.142$ \\
% SDXL w/o object cues & $2.601 \pm 2.906$ & $0.891 \pm 0.011$ & $5.649 \pm 15.050$ & $37.809\%$ & $0.761 \pm 0.284$ \\
% SDXL w/o prompts & $3.555 \pm 2.374$ & $0.988 \pm 0.001$ & $5.798 \pm 15.107$ & $37.374\%$ & $0.757 \pm 0.285$ \\
% \hline
% \end{tabular}
% \caption{Comparison of metrics across different SDXL 2D methods: with object prompts, no cues, and no prompts for the \nyu dataset.}
% \label{table:SDXL_ablations_2D_NYU}
% \end{table*}


% %%%%%%%%%%%%% Outpainting 2.5D
% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% SDXL w/ object cues    & $1.752 \pm 2.043$ & $0.617 \pm 0.305$ & $6.277 \pm 2.229$ & 0.00\% \\
% SDXL w/o object cues   & $1.833 \pm 2.011$ & $0.886 \pm 0.104$ & $18.144 \pm 6.148$ & 55.409\% \\
% SDXL w/o prompts        & $1.874 \pm 1.988$ & $0.931 \pm 0.016$ & $18.533 \pm 9.178$ & 58.927\% \\
% \hline
% \end{tabular}
% \caption{Comparison of metrics across different SDXL 2.5D methods: with object prompts, no cues, and no prompts for the \rk dataset.}
% \label{table:SDXL_Re10k_2.5D}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% SDXL w/ object cues    & $1.533 \pm 2.916$ & $0.655 \pm 0.323$ & $5.245 \pm 2.351$ & 0.00\% \\
% SDXL w/o object cues   & $2.612 \pm 1.398$ & $0.818 \pm 0.102$ & $12.637 \pm 9.184$ & 37.809\% \\
% SDXL w/o prompts        & $2.807 \pm 1.616$ & $0.987 \pm 0.010$ & $16.998 \pm 7.356$ & 37.374\% \\
% \hline
% \end{tabular}
% \caption{Comparison of metrics across different SDXL 2.5D methods: with object prompts, no cues, and no prompts for the \nyu dataset.}
% \label{table:SDXL_NYU_2.5D}
% \end{table*}


% %%%%%%%%%%%%% 3D

% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% DFM ($n_{s}=25, k=4$) & $2.471 \pm 4.415$ & $0.303 \pm 0.202$ & $9.190 \pm 6.223$ & $1.740\%$ \\
% DFM ($n_{s}=25, k=3$) & $2.774 \pm 7.210$ & $0.412 \pm 0.201$ & $10.344 \pm 7.004$ & $4.122\%$ \\
% DFM ($n_{s}=25, k=2$) & $4.102 \pm 4.815$ & $0.508 \pm 0.210$ & $12.001 \pm 7.350$ & $32.125\%$ \\
% \midrule
% DFM ($n_{s}=15, k=4$) & $3.718 \pm 4.950$ & $0.821 \pm 0.202$ & $11.210 \pm 6.702$ & $6.450\%$ \\
% DFM ($n_{s}=10, k=4$) & $3.210 \pm 3.550$ & $0.965 \pm 0.050$ & $13.105 \pm 7.219$ & $18.370\%$ \\
% \hline
% \end{tabular}
% \caption{3D Ablation study of DFM with different configurations of $n_s$ and $k$ on the \rk dataset.}
% \label{table:DFM_3D_ablation_Re10k}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{Methods} & $\cent\downarrow$ & $\ent\downarrow$ & $\dnn(\%)\downarrow$ & $\falseneg \downarrow$ \\
% \hline
% DFM ($n_{s}=25, k=4$) & $2.062 \pm 3.915$ & $0.541 \pm 0.374$ & $3.948 \pm 5.801$ & $0.000\%$ \\
% DFM ($n_{s}=25, k=3$) & $3.876 \pm 6.235$ & $0.768 \pm 0.426$ & $6.572 \pm 6.245$ & $13.765\%$ \\
% DFM ($n_{s}=25, k=2$) & $6.125 \pm 7.325$ & $0.983 \pm 0.492$ & $9.815 \pm 7.412$ & $45.320\%$ \\
% \midrule
% DFM ($n_{s}=15, k=4$) & $4.521 \pm 5.813$ & $0.912 \pm 0.628$ & $8.210 \pm 6.925$ & $8.413\%$ \\
% DFM ($n_{s}=10, k=4$) & $6.832 \pm 3.750$ & $0.965 \pm 0.702$ & $11.582 \pm 7.625$ & $28.765\%$ \\
% \hline
% \end{tabular}
% \caption{3D Ablation study of DFM with different configurations of $n_s$ and $k$ on the \nyu dataset.}
% \label{table:DFM_3D_ablation_NYU}
% \end{table*}

    % % Row 8
    % \rotatebox[origin=l]{90}{{\footnotesize LAPTOP}}
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \begin{tikzpicture}
    %         \node [anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=\linewidth]{heatmaps/640x360_living_room_0016_1300200232.988284-1300278508.png}};
    %         \draw[white, thick, dashed] (0.22*\linewidth, 0.01) -- (0.22*\linewidth, 0.5648*\linewidth);
    %         \draw[white, thick, dashed] (0.78*\linewidth, 0.01) -- (0.78*\linewidth, 0.5648*\linewidth);
    %     \end{tikzpicture}
    %     \label{fig:qual_r8_col1}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.152\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{heatmaps/NYU_6_laptop_output_heatmap.png}
    %     \label{fig:qual_r8_col2}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{SDXL_maps/laptop_heatmap_image.png}
    %     \label{fig:qual_r8_col3}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{gpt/laptop_16.png}
    %     \label{fig:qual_r8_col4}
    % \end{subfigure}\\
    % \vspace{-1em}
     % Row 9
    % \rotatebox[origin=l]{90}{{\footnotesize LAPTOP}}
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \begin{tikzpicture}
    %         \node [anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=\linewidth]{heatmaps/640x360_living_room_0016_1300200232.988284-1300278508.png}};
    %         \draw[white, thick, dashed] (0.22*\linewidth, 0.01) -- (0.22*\linewidth, 0.5648*\linewidth);
    %         \draw[white, thick, dashed] (0.78*\linewidth, 0.01) -- (0.78*\linewidth, 0.5648*\linewidth);
    %     \end{tikzpicture}
    %     \label{fig:qual_r9_col1}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.152\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{heatmaps/NYU_6_laptop_output_heatmap.png}
    %     \label{fig:qual_r9_col2}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{SDXL_maps/laptop_heatmap_image.png}
    %     \label{fig:qual_r9_col3}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{gpt/laptop_16.png}
    %     \label{fig:qual_r9_col4}
    % \end{subfigure}\\
    % % Row 10
    % \rotatebox[origin=l]{90}{{\footnotesize LAPTOP}}
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \begin{tikzpicture}
    %         \node [anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=\linewidth]{heatmaps/640x360_living_room_0016_1300200232.988284-1300278508.png}};
    %         \draw[white, thick, dashed] (0.22*\linewidth, 0.01) -- (0.22*\linewidth, 0.5648*\linewidth);
    %         \draw[white, thick, dashed] (0.78*\linewidth, 0.01) -- (0.78*\linewidth, 0.5648*\linewidth);
    %     \end{tikzpicture}
    %     \label{fig:qual_r10_col1}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.152\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{heatmaps/NYU_6_laptop_output_heatmap.png}
    %     \label{fig:qual_r10_col2}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{SDXL_maps/laptop_heatmap_image.png}
    %     \label{fig:qual_r10_col3}
    % \end{subfigure}\hfill
    % \begin{subfigure}[]{0.27\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{gpt/laptop_16.png}
    %     \label{fig:qual_r10_col4}
    % \end{subfigure}\\
    
% We observe that sometimes the model correctly ignores the prompt witht he object cues in cases where an object is cues incorrectly as in \cref{fig:ignored_microwave}.
% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{living_room_0016_1300200232.988284-1300278508_target_laptop_outpainted_Extend_the_scene_with_the_object__microwave_7.5_2021_0.jpg}
%     \caption{SDXL model ignores the cue of a oven for the given context image.}
%     \label{fig:ignored_microwave}
% \end{figure}





% This limitation highlights the need to extend the analysis to the synthetic domain, where access to a true distribution is available.

% \paragraph{Future work.}
% However, the task necessitates that the detection pipelines do not overfit to align with the ground truth realizations, which notably is \textit{not} the true (unavailable) conditional distribution. 
% Dylan: We can't really distinguish between the overfit case (=oracle) and the true distribution with our metrics, so we are relying on the model not being able to overfit to the test set. A long way of saying, this isn't helpful here, but could be a reasonable point to make in the discussion later.
% This is the motivation for the synthetic experiments in your next project.

% Future work can study task performance in controlled synthetic benchmarks where the true conditional distribution might be made available.

% Finally, future work could explore how \task interacts with downstream tasks, such as robot reactive control~\citep{react} to choose between going forward, left, or right, where coarse-grained spatial resolutions are likely to be sufficient, or visual search~\citep{vsearch} and long-horizon probabilistic planning~\citep{kurniawati2022partially}, where relatively fine-grained spatial resolutions may be needed. 
% \Task can pave the way for a richer understanding of detection uncertainty~\citep{pod}, recovering semantic relations such as affordances~\citep{saycan}, enabling adaptive planning~\citep{jutrasdube2024adaptive} and navigation~\citep{shah2023vint}.









% in uncertain environments~\citep{auto}.


% This study has several limitations. High inference times, particularly with 3D diffusion models, challenge real-time robotic applications, as numerous samples are needed to approximate the conditional distribution. 
% The reliance on object prompts in outpainting methods may introduce bias, while evaluations using vision-language models (VLMs) risk unreliability; these pre-trained, closed models might have been exposed to test images, leading to potential memorization. Our method detects objects identifiable by models like YOLOv8x~\citep{ultralytics2023yolov8}, which may differ from human perception, indicating a need for models that generate samples directly from conditional SSDs, focusing on diversity over photorealism. The trade-off between generation quality and diversity~\citep{pareto} raises questions about the importance of fidelity and geometric consistency in generation; prioritizing diversity may better align with \task's goals. While pre-trained generative models produced promising results, task-specific training could further improve accuracy.

% The 2D, 2.5D, and 3D domains identify key challenges in \task.
% Extending the camera frame enables the prediction of objects beyond the visible frustum in both 2D and 3D. The 2.5D representation balances local depth and occlusion cues with spatial understanding, bridging 2D and 3D without needing full scene reasoning. 
% Only the 3D pipelines can estimate fully occluded objects by reasoning 
% beyond visible surface.

% This work introduces \task across 2D, 2.5D, and 3D domains, assessing detection pipelines on indoor scenes and common objects to identify key differences. 
% outside the frustum, 
% while 2D methods using outpainting and vision-language models cannot handle occlusions. 
% 3D diffusion models handle occlusions more effectively, showcasing \task's potential to enhance spatial reasoning in autonomous systems.

% Future work will target faster inference through task-specific training that skips intermediate steps, enhancing robotic capabilities in policy improvement, reactive planning, visual search, navigation, and long-horizon planning in new environments~\citep{spartn, react, vsearch, vsn, nav_real, dimsam, safe, carvalho2024motion, longhorizon}. Coarse resolutions may suffice for reactive tasks, while finer resolutions could support visual search and planning. To accelerate inference, one could generalize 3D modeling to panoramic image outpainting~\citep{wu2023panodiffusion} and depth estimation in such domain to be lifted in 3D~\citep{panodepth}, providing results comparable to 3D diffusion models. Finally, examining how specific objects and their spatial and label uncertainties~\citep{pod} shape SSDs could yield insights into causal relations within learned representations of generative models~\citep{Scholkopfetal21, causal}.

% \paragraph*{Acknowledgment.} 


% This study has several limitations. The inference time of generative models, particularly 3D diffusion models, is high, posing challenges for real-time robotics. Our reliance on many samples to approximate the conditional distribution can create a bottleneck. 
% Additionally, the dependence on object prompts in outpainting-based methods may introduce bias. Evaluations with VLMs may also be unreliable, as these closed, pre-trained models could have been exposed to test images during training, risking memorization. 
% Our approach produces detections recognized by models like YOLOv8x~\citep{ultralytics2023yolov8}, even if human perception might differ. This prompts the need for models generating samples directly from conditional SSDs, prioritizing diversity over photorealism. \rudra{Given that higher quality trade off with diversity in generation~\citep{pareto}, it remains unclear whether high-fidelity or geometric consistency is necessary for the generation, as prioritizing diversity may be more important for \task.} While pre-trained generative models yielded promising results, task-specific training are expected to further improve accuracy. 
% Finally, our findings rekindle questions about causal relations in learned representations~\citep{causal} and the implications of model choices in representation learning.



% This work introduces \task across 2D, 2.5D, and 3D, presenting three detection pipelines evaluated on indoor scenes and common objects. We identify key differences between 2D and 3D tasks. Expanding the camera frame is effective in both, with pipelines predicting objects outside the visible frustum. 
% The 2.5D representation offers a balance by capturing local depth cues and occlusion awareness, bridging 2D perception with 3D understanding while efficiently encoding spatial structures without requiring global scene reasoning. In contrast, 3D pipelines excel in detecting fully occluded objects, reasoning beyond the camera frustum. While 2D pipelines based on outpainting and VLMs struggle with occlusions, 3D diffusion models demonstrate superior occlusion handling, reflecting \task’s potential.

% \rudra{Future work will explore task-specific training to bypass intermediate generation stages and address bottlenecks, thereby optimizing for real-time inference. This could further enable applications in robotics such as improving policies~\citep{spartn}, reactive planning~\citep{react}, visual search~\citep{vsearch}, navigation~\citep{vsn, nav_real}, task and motion planning~\citep{dimsam, safe, carvalho2024motion}, and long-horizon planning in unseen environments~\citep{longhorizon}. More advanced end-to-end models could capture spatial and label uncertainty of detection within the generative process using maximum likelihood estimation and training~\citep{pod, mle}.}\rudra{Please have a discussion before updating this.}

% While the work presents a promising initial step towards this significant task, it also sets up some open questions. 
% For example, while all of the detection pipelines presented in this work use pre-trained generative models, 
% it is likely that training for this task directly would elicit more accurate predictions. 
% Moreover, the 2D and 3D diffusion
% models are repurposed from their original task of photorealistic generation, 
% but it is unclear whether high-fidelity
% generation is desirable for unobserved object detection. 
% One might expect it to be simpler to train a model to directly generate samples from the conditional SSD at lower resolutions. 
% Finally, future work could explore how unobserved object detection interacts with downstream tasks, such as robot reactive control to choose between going forward, left, or right, where coarse-grained spatial resolutions are likely to be sufficient, 
% or visual search and long-horizon probabilistic planning, 
% where relatively fine-grained spatial resolutions may be needed.
% \rudra{Finally, future work could investigate how the presence of specific objects within an image influences the SSD of other contextually aligned objects, advancing our understanding of causal object relationships within learned representations~\citep{Scholkopfetal21, causal}.}



% \subsubsection*{Ethical and Environmental Considerations, System Requirements, and Reproducibility.}
% Our \task approach aims to improve autonomous reasoning with potential societal benefits. 
% \rudra{However, inferring beyond observations presents risks, such as privacy breaches and biased outcomes due to uneven training data in pre-trained models.} 
% However, the use of pre-trained models presents risks such as datasets compromised by privacy sensitive information or implicit biases.  
% In the current work we take steps to mitigate some privacy considerations by excluding scenes with people.
% We minimize environmental impact by using pre-trained models, public datasets, and APIs while optimizing resource use. 

==> sections/progress.tex <==
\section{Current Progress, Timeline \& Further Work}

In this report, we summarize the progress made so far in our investigation of Unobserved Object Detection and outline the planned next steps until the end of September 2025.

\subsection{Summary of Progress}
\begin{enumerate}
    \item[\tick] Developed the initial probabilistic framework for unobserved object reasoning.
    \item[\tick] Implemented a baseline generative model for spatial-semantic inference.
    \item[\untick] Evaluated uncertainty quantification methods on synthetic and procedurally generated datasets by training and sampling our model, using metrics developed when a non-singular ground truth distribution is available.
    \item[\untick] Tested the framework’s applicability in real-world environments using robots equipped with cameras post-retraining, including derived models such as occupancy models.
\end{enumerate}

\subsection{Timeline of Progress Since TPR and Future Work}
\begin{enumerate}
    \item \textbf{March -- May 2024 (Post-TPR)}: Perform sequential sampling of the DFM to assess the feasibility of the process.
    \item \textbf{June -- July 2024}: Develop ground truth distributions and establish baseline models.
    \item \textbf{August 2024}: Create and validate evaluation metrics alongside SDXL baselines.
    \item \textbf{September 2024}: Conduct an extensive study of Vision-Language Models (VLMs) and adapt the metrics for this task.
    \item \textbf{October 2024}: Extend the framework to incorporate NYU datasets.
    \item \textbf{November 2024}: Write, polish, and submit the paper; internship begins mid-November.
    \item \textbf{March 2024 -- May 2025}: 
    \begin{enumerate}
        \item Evaluate uncertainty quantification on synthetic and procedurally generated datasets; iterate on model improvements based on experimental outcomes.
        \item Test the framework in real-world scenarios using robots with cameras to assess probabilistic modeling of real-world occupancy.
    \end{enumerate}
    \item \textbf{June 2025}: Develop the formulation for the synthetic dataset conditional distribution problem by defining conditional distributions and establishing evaluation criteria.
    Implement the conditional distribution model on the synthetic dataset and run preliminary experiments to assess performance.
    \item \textbf{July 2025}: Find connections to robotic applications which can directly use the generated distribution in a simulated setting, motivating our use case for robotics.
    \item \textbf{August -September 2025}: Conduct extensive experiments, refine results, and push for submission to ICLR / ICRA or other major AI/Robotics conferences in 2026.
\end{enumerate}

\section{Task Summary: Unobserved Object Detection}
Can objects that are not visible in an image---but are in the vicinity of the camera---be detected?
This study introduces the novel tasks of 2D, 2.5D and 3D unobserved object detection for predicting the location of nearby objects that are occluded or lie outside the image frame. 
We adapt several state-of-the-art pre-trained generative models to address this task, including 2D and 3D diffusion models and vision--language models, and show that they can be used to infer the presence of objects that are not directly observed. 
To benchmark this task, we propose a suite of metrics that capture different aspects of performance. 
Our empirical evaluation on indoor scenes from the \rk and \nyu datasets demonstrate results that motivate the use of generative models for the unobserved object detection task.

